Reaching the intrinsic performance limits of superconducting nanowire single-photon detectors up to 0.1 mm wide

Superconducting nanowire single-photon detectors (SNSPDs) combine high detection efficiency, low noise, and excellent timing resolution, making them a leading platform for photon-counting applications. However, despite decades of materials and fabrication research, detector performance has never been shown to match theoretical performance expectations. Here, we demonstrate for the first time in situ tuning of a detector from its typical, suboptimal operation, to a regime limited only by material quality, allowing the device to reach its intrinsic performance limit. Our approach is based on current-biased superconducting "rails" placed on either side of the detector that redistribute current across its width to achieve its peak performance. This technique reduces the dark count rate by ten orders of magnitude. Further, we show operation at this intrinsic performance limit for devices up to 0.1 mm wide, and also demonstrate near-unity internal detection efficiency (IDE) at a wavelength of 4um for a 20um-wide detector--a factor of 20 wider than the current state of the art. This work enables future detectors to overcome the Pearl limit for device width, paving the way for arbitrarily large detectors.

==> supplementary_body_old.tex <==
\section{Methods}\label{secA1}
\subsection{{Fabrication}}
The chips were fabricated with 5 layers: 1 WSi layer, 1 Nb layer, 1 Au layer and 2 dielectric (SiO2) spacer layers. First, we sputter a $\approx 3$~nm-thick film of WSi on a 75~mm silicon wafer with 150~nm of thermal oxide. The film was capped with $\approx 2$~nm $\alpha$Si to prevent oxidation. Next we patterned our wires using ZEP520A using electron-beam lithography. Then the film was etched using an inductively coupled plasma-reactive ion etcher (ICP-RIE) and an AR:SF6 etch. 

For the next layer, we pattern LOR3A + SPR660 using photolithography for the dielectric spacer layer. We sputter $\approx 25$~nm SiO2 and liftoff the resist---this layer isolates the WSi wire from the Nb rails. Then, we pattern LOR3A + SPR660 using photolithography for Nb liftoff. We then sputter $\approx 50$~nm of Nb and lift it off. Next, we pattern our rails using ZEP520A using electron-beam lithography. The Nb is etched using the ICP-RIE and an SF6 etch.

For the next layer, we pattern LOR3A + SPR660 using photolithography for the dielectric spacer layer. We sputter $\approx 25$~nm SiO2 and liftoff the resist---this layer isolates the Nb rails from the Au covers. Then we pattern taper covers in LOR3A + SPR660 using photolithography for Au liftoff. We evaporate $\approx 100$~nm Au and lift it off. 

\subsection{Verification of unity internal detection efficiency}\label{secA2}
As noted in Fig~2(a) in the main text, a slope on our detection plateau was evident for uncovered detectors of all widths. We hypothesize that this slope is a result of our experiments being performed under flood illumination causing detection events in the taper of our devices as has has been noted in previous studies~\cite{chiles2020superconducting}. To test this hypothesis, we fabricated several devices with gold covers placed over the taper in order to block light from hitting the tapers. In these gold covered devices, the only region expossed to light should be the uncovered portion of the constriction. In Fig~1(e) in the main text, we show an example of results obtained using a 50~$\mu$m device with a gold cover. The gold cover has a 10~$\mu$m-long opening over the center of the constriction. Here the slope appears to be completely eliminated by the addition of the cover. In the case of the 100~$\mu$m-wide SNSPDs with gold covers, we do not measure a complete reduction in plateau slope. Further study is needed to determine the cause of this discrepancy. 

We also verified unity internal detection efficiency using a focused beam spot on a 20~$\mu$m-wide SNSPD. Here we measured the photon count rate on the plateau as a function of rail current and found less than 1\% variation in the count rate over the range of rail current studied here.


\section{Field and current in the rail SNSPD}\label{secS1}
%\numberwithin{equation}{section}

Consider a long thin film wire of width $w$ situated at $y=0$ between two thin film rails of width $l$ at $w/2+b<x<w/2+b+l$ and $-w/2-b-l<x<-w/2-b$, as shown in Fig.~\ref{figD1}. Here each rail is raised by the height $h$ and spaced by $b$ from the edge of the wire. It is assumed that the wire carries a dc current $I_s$ and each rail carries a dc current $I_r$, both the wire and the rails are infinite along $z$. 

\begin{figure}[h]
\centering
   	\includegraphics[scale=0.6,trim={0mm 0mm 0mm 0mm},clip]{supplementary/A1.pdf}
   	\caption{Geometry of a detector film of width $w$ and two current rails of width $l$. The coordinate axes are shifted downward for clarity.}
   	\label{figD1}
   \end{figure}

In this geometry the $z$-component of magnetic field $B_z$ along the wire vanishes and other field components $B_x=\partial A/\partial y$ and $B_y=-\partial A/\partial x$ are expressed in terms of the $z$ component of the vector potential ${\bf A}(x,y)=[0,0,A(x,y)]$ caused by currents flowing along $z$. Here $A(x,y)$ satisfies the London equation:
\begin{equation}
\lambda^2\nabla^{2}A-dQ(x)\delta(y)=0,
\label{D1}
\end{equation}
where the gauge-invariant ${\bf Q}={\bf A}+(\phi_{0}/2\pi)\nabla\theta$ is proportional to the supercurrent density ${\bf j}=-{\bf Q}/\mu_0\lambda^2$ in the film,  $\theta$ is the phase of the superconducting order parameter, $\phi_0$ is the magnetic flux quantum, $\lambda$ is the London penetration depth, $d$ is the film thickness. In the planar geometry considered here $j_x=j_y=0$, $j_z(x)$ is flowing along the wire length and the rail current can depend only on $x$, so the phase gradients $\nabla\theta=(0,0,\theta')$ have only a constant z-component $\theta'$ independent of $x$. We consider here films with $d\ll\lambda$ in the absence of vortices and $Q\ll \phi_0/2\pi\xi$ for which the linear London electrodynamics is applicable, where $\xi$ is a coherence length. The solution of Eq.~(\ref{D1}) is given by: 
\begin{gather}
A(x,y)=\frac{d_sw}{8\pi\lambda_s^{2}}\int_{-1}^{1}\ln[(x-u)^{2}+y^{2}]Q_s(u)du+
\label{D2} \\ 
\frac{d_rw}{8\pi\lambda_{r}^{2}}\biggl[\int_{1+b}^{1+b+l}\!\!\!\ln[(x-u)^{2}+(y-h)^{2}]Q_{r}(u)du+\int_{-1-b-l}^{-1-b}\!\!\!\ln[(x-u)^{2}+(y-h)^{2}]Q_{r}(u)du\biggr],
\nonumber
\end{gather}
where $Q_s(x)$ and $Q_r(x)$ determine the supercurrent densities in the wire and the rails, respectively. Here $\lambda_s$ and $\lambda_r$ are the London penetration depths in the wire and the rails, $d_s$ and $d_r$ are their respective thicknesses, and all lengths are in units of $w/2$. Using $Q_s(u)=Q_s(-u)$ and $Q_{r}(u)=Q_{r}(-u)$ reduces Eq.~(\ref{D2}) to
\begin{gather} 
A(x,y)=k_s\int_{0}^{1}\ln[((x-u)^{2}+y^{2})((x+u)^{2}+y^{2})]Q_s(u)du+
\nonumber \\
k_r\int_{1+b}^{1+b+l}\ln[((x-u)^{2}+(y-h)^{2})((x+u)^{2}+(y-h)^{2})]Q_{r}(u)du,
\label{D3} 
\end{gather}
where $k_s=w/4\pi\Lambda_s$, $k_r=w/4\pi\Lambda_r$, and $\Lambda_s=2\lambda_s^2/d_s$ and $\Lambda_r=2\lambda_r^2/d_r$ are the Pearl screening lengths in the wire and rails, respectively. Setting $y=0$ in Eq.~(\ref{D3}) and using $A(x,0)=Q(x,0)-\phi_0\theta'/2\pi$ gives two equations for $Q_s(x)$ and $Q_r(x)$:
\begin{gather}
\!\!\!Q_s(x)-2k_s\!\!\int_0^1\!\ln|x^{2}-u^{2}|Q_s(u)du-k_{r}\!\!\int_{1+b}^{1+l+b}\!\!\ln[(u^{2}+h^{2}-x^{2})^{2}+4h^{2}x^{2}]Q_{r}(u)du=\alpha,
\label{D4} \\
\!\!\!Q_r(x)-2k_{r}\!\!\int_{1+b}^{1+b+l}\!\!\ln|x^{2}-u^{2}|Q_{r}(u)du-k_{s}\!\!\int_0^1\!\ln[(u^{2}+h^{2}-x^{2})^{2}+4h^{2}x^{2}]Q_s(u)du=\beta,
\label{D5}
\end{gather}
where $\alpha=\phi_{0}\theta_s'/2\pi$ and $\beta=\phi_0\theta_r'/2\pi$ with constant phase gradients $\theta'_s$ and $\theta_r'$.

Equations~(\ref{D4}) and (\ref{D5}) were solved by discretizing $u_n=s(n-1)$, $n=1,... N_1$ and introducing a vector $Q=(Q_1,Q_2..., Q_{N_1})$ which includes $Q_s(sn)$ at $1<n<N$ and $Q_r(sn)$ at $N+1<n<N_1$ with $s=1/(N-1)$, $N_1=[(1+l)N]$ and $N=6\cdot 10^3$. As a result, Eqs.~(\ref{D4}) and (\ref{D5}) take the matrix form:
\begin{equation}
\sum_m M_{nm}Q_m=\alpha_n,\qquad Q_n=\sum_mM^{-1}_{nm}\alpha_m.
\label{D6}
\end{equation}
Here $M_{nm}$ defined by Eqs.~(\ref{D4}) and (\ref{D5}) is given below, $\alpha_n=\alpha$ at $1<n<N$ and $\alpha_n=\beta$ at $N+1<n<N_1$. To express $\alpha$ and $\beta$ in terms of currents $I_s=(4s/\mu_0\Lambda_s)\sum_{n=1}^NQ_n$ and $I_r=(2s/\mu_0\Lambda_r)\sum_{n=N+1}^{N_1}Q_n$, we sum up the second Eq.~(\ref{D6}) over $n$ using that $\alpha_m$ are constants at $1<m<N$ and $N+1<m<N_1$ and obtain:
\begin{gather}
I_s=A\alpha +B\beta,\qquad I_r=A_1\beta +B_1\alpha.
\label{D7}
\end{gather}
Hence,
\begin{gather}
\alpha=\frac{A_1I_s-BI_r}{AA_1-BB_1}, \qquad \beta=\frac{AI_r-B_1I_s}{AA_1-BB_1},
\label{D8}
\end{gather}
where
\begin{gather}
A=\frac{4s}{\mu_0\Lambda_s}\sum_{n=1}^N\sum_{m=1}^NM_{nm}^{-1},\qquad B=\frac{4s}{\mu_0\Lambda_s}\sum_{n=1}^N\sum_{m=N+1}^{N_1}M_{nm}^{-1},
\label{D9}\\
A_1=\frac{2s}{\mu_0\Lambda_r}\sum_{n=N+1}^{N_1}\sum_{m=N+1}^{N_1}M_{nm}^{-1},\qquad B_1=\frac{2s}{\mu_0\Lambda_r}\sum_{n=N+1}^{N_1}\sum_{m=1}^{N}M_{nm}^{-1}.
\label{D10}
\end{gather}
The matrix elements $M_{nm}$ are given by
\begin{gather}
M_{nm}=\delta_{nm}-2k_ss\ln|(n^2-m^2)s^2|,\quad 1<n<N,\,\, 1<m<N,
\nonumber \\ 
M_{nm}=-k_rs\ln[((ms+b)^{2}-n^2s^2+h^2)^2+(2hns)^2],\quad 1<n<N,\,\, N+1<m<N_1,
\nonumber \\
M_{nm}=-k_ss\ln[((ns+b)^2-m^2s^2+h^2)^2+(2hms)^2],\quad N+1<n<N_1,\,\, 1<m<N,
\nonumber \\
M_{nm}=\delta_{nm}-2k_rs\ln|(ns+b)^2-(ms+b)^2|,\quad N+1<n<N_1,\,\, N+1<m<N_1.
\nonumber
\end{gather}
The logarithmic singularity in $M_{nn}$ was integrated out: $M_{nn}\to 1- 2sk_s[\ln(s/2)-1+\ln(2sn)]$ and 
$M_{nn}\to 1- 2sk_r[\ln(s/2)-1+\ln(2sn+2b)]$. Reduction of the sheet current density $J(x)=d_sj_s(x)$ at the edges comes from off-diagonal elements of $M_{nm}$ accounting for the inductive coupling of the rails and SNSPD. Examples of $J(x)$ in wires of different widths calculated from Eqs.~(\ref{D4}) and (\ref{D5}) are shown in Fig.~1(a) in the main text and Fig.~\ref{figD2}. Particularly, Fig.~\ref{figD2}(b) shows that the rail-controlled reduction of $J(x)$ at the edges can be achieved in a wire 4 times wider than the Pearl length. For $\Lambda\approx 600\,\mu$m for our WSi films, Fig.~\ref{figD2}(b) corresponds to a 2.5~mm-wide wire. After $Q_s(x)$ and $Q_r(x)$ have been obtained, the magnetic field around the SNSPD-rail is calculated using Eq.~(\ref{D2}), as shown in Fig.~1(a) in the main text.  

\begin{figure}[h]
   	\includegraphics[scale=0.35,trim={5mm 0mm 0mm 0mm},clip]{supplementary/Fa.pdf}
	\includegraphics[scale=0.35,trim={10mm 0mm 0mm 0mm},clip]{supplementary/Fb.pdf}
   	\caption{Sheet current density $J(x)$ in the central wire calculated at different normalized rail currents $I_r/I_s$ for WSi films with $d_s=3$~nm, $\Lambda_s = 602\,\mu$m, $k_r=200k_s$, $l=0.15w$ and $b=0.005w$:  (a) $w\approx 50\,\mu$m, $I_r/I_s= 0.62, 1.89, 3.15,  4.81$ (b) $w\approx 2.5$~mm, $I_r/I_s=0.32, 0.41, 0.51, 0.65$.}
   	\label{figD2}
   	\end{figure}
%\setcounter{figure}{0}

\section{Energy barriers and dark count rates caused by vortices}\label{secS2}

% \numberwithin{equation}{section}

The position-dependent energy of a vortex $E(x)$ in a thin film of width $w\ll \Lambda_s$ calculated in the London model is given by~\cite{gurvink}:
\begin{equation}
E(x)=\epsilon\ln\left(\frac{w}{\pi\tilde{\xi}}\sin\frac{\pi x}{w}\right)-\phi_{0}J_sx,
\label{E1}
\end{equation}
where $\epsilon=\phi_{0}^{2}/2\pi\mu_{0}\Lambda_s$ is the vortex line energy, the numerical factor in $\tilde{\xi}\approx 0.34\xi_s$ accounts for the vortex core energy, and $J_s$ is a uniform sheet current density. The maximum in $E(x)$ occurs at $x=x_m$, where:
\begin{equation}
x_m=\frac{w}{\pi}\cot^{-1}\frac{J_s}{J_{0}},\qquad J_{0}=\frac{\pi\epsilon}{\phi_{0}w}=\frac{\phi_{0}}{2\mu_{0}w\Lambda_s}\sim\frac{\xi_s}{w}J_{d}\ll J_{d}.
\label{E2}
\end{equation}
The London model with a point vortex core is applicable for a wide wire with $w\sim (10^2-10^3)\xi_s$, but becomes invalid for a vortex spaced by $\sim \xi_s $ from the edges. Here $E(x)$ given by Eq.~(\ref{E1}) diverges logarithmically at $x\to 0$, whereas the energy of a vortex emerging from the wire edge vanishes. Numerical calculations of $E(x)$ using the Ginzburg-Landau equations~\cite{Vodolaz} have shown that the London model describes $E(x_m)$ well if $J_s$ is not too close to $J_d$ and the energy barrier at $J_s=J_d$ vanishes.  To take this effect into account, we define the energy barrier for the vortex entry as $U=E[x_m(J)]-E[x_m(J_d)]$, where $E(x)$ and $x_m$ are given by Eq.~(\ref{E1}) and (\ref{E2}). At $J_s\gg J_0$ this yields the energy barrier independent of the film width:
\begin{equation}
U=\epsilon\ln (J_d/J_s),\qquad J_s\gg J_d\xi/w.
\label{E3}
\end{equation}
This gives a reasonable estimate of $U(J)$ at $J_s\simeq J_d$ at which $x_m\sim \xi_s\ll w$ shifts close to the edge of the film, as depicted in Fig. \ref{figE1}. 
Thermally-activated hopping of vortices over the edge barrier results in a mean dc voltage     
$V =V_0(J_s/J_d)^{\epsilon/T}$, where $V_0$ was evaluated in Ref.~\cite{gurvink}. At $\epsilon/T\gg1$ and $J_s\simeq J_{d}$ the V-I curve  takes the form: 
\begin{equation}
V=V_0\exp[-U/T],\qquad U\simeq\epsilon(1-J_s/J_d).
\label{E4}
\end{equation}
For our 3~nm thick WSi films with $\lambda=950$~nm and $\Lambda\approx600\,\mu$m, we get $\epsilon\simeq 66$~K. At $J_s=0.9J_{d}$ and $T=0.9$~K the probability of thermally-activated penetration of a vortex from an ideal film edge is proportional to the small Arrhenius factor $\propto\exp(-U/T)\sim 7\cdot10^{-4}$ which can increase substantially due to edge defects which locally reduce the energy barrier and facilitate penetration of vortices.
\begin{figure}[h]
\centering
   	\includegraphics[scale=0.4,trim={0mm 0mm 0mm 0mm},clip]{supplementary/bara.pdf}
   	\caption{Qualitative dependence of $E(x)$ on the vortex position evaluated from Eqs. (\ref{D1}) regularized by $x\to\tilde{x}= [x^2+\tilde{\xi}^2]^{1/2}$, $E(x)\to E(\tilde{x})+\phi_0J_s\tilde{\xi}$, $\tilde{\xi}=10^{-2}w$ and $J_s=20J_0$. }
   	\label{figE1}
   	\end{figure}
Edge defects can be small indentations or other microstructural features causing local variations of $T_c$ or current crowding around defects. For instance, the local current density at the edge of a semicircular indentation of radius $R\gg\xi$ is twice the mean $J_s$, and larger concentration of impurities at the edges causes local reduction of $J_d$. Such defects serve as gates for local penetration of vortices for which the energy barrier $U(J_s)$ vanishes at the mean current density $\bar{J}_d$ smaller than the bulk $J_d$. Given many material uncertainties depending on the film growth and deposition parameters, we assume that edge imperfections locally reduce the mean depairing density to $\tilde{J}_d<J_d$ in a narrow strip along the edges. It is the reduction of $\tilde{J}_d$ at the edge which is mitigated by the current rails. With that in mind, consider now the number $S_e$ of thermally-activated vortices penetrating over the edge barrier per unit time in a film of length $L$:
\begin{equation}
S_e = S_{e0}\exp\biggl[-\frac{\epsilon}{T}\left(1-\frac{J_s}{\tilde{J}_d}\right)\biggr],\qquad S_{e0}\sim \frac{L\nu}{l_i}.
\label{E5} 
\end{equation}
Here $L/\l_i$ is a number of statistically-independent vortex entries through edge defects with a mean spacing $l_i$ and $\nu$ is an attempt frequency. In the overdamped limit characteristic of Abrikosov vortices, $\nu\simeq \sqrt{k_ak_b}/4\pi\eta$ follows from the classical result of Kramers~\cite{kramers}, where $k_a$ and $k_b$ are curvatures of $E(x)$ at the bottom and the top of the potential well depicted in Fig.~\ref{figE1}, $\eta=\phi_0^2d_s/2\pi\xi^{2}\rho_n$ is the Mattis-Bardeen vortex drag coefficient, and $\rho_n$ is the normal state resistivity.  Taking $\sqrt{k_{a}k_{b}}\sim \phi_{0}^{2}d_s/4\pi\mu_{0}\lambda_s^2\xi_s^{2}$ at $J_s\sim \tilde{J}_d$ in Eq.~(\ref{E5}) yields
\begin{equation}
S_{e0}\sim \frac{L\rho_n}{8\pi\mu_0\lambda_s^2 l_i}.
\label{E6}
\end{equation}
For a WSi film with $L=0.1$~mm, $\lambda=950$~nm, $\rho_n=2.5\,\mu\Omega$m and $l_i\sim 10^2$~nm, we get $S_{e0}\sim 10^{12}$ s$^{-1}$. Here Eq.~(\ref{D6}) is a rough, order of magnitude estimate which takes into account neither microstructural details of edge imperfections nor deformation of the vortex core at the edge in the presence of current~\cite{Vodolaz}. The latter can result an extra factor $(1-J_s/J_d)^n$ with $n=1-2$, yet the logarithmic slope 
\begin{equation}
\frac{d\ln S_{e}}{dJ_s}=\frac{\epsilon}{T\tilde{J}_d} 
\label{E7}
\end{equation}
is practically insensitive to uncertainties in $S_{e0}$ and its possible power-law dependence on $J_s$ if $T\ll\epsilon$.  

From Eq.~(\ref{E5}), we obtain a maximum current $I_{c1}$ which the SNSPD can carry at a given dark count rate $S_c$:
\begin{equation}
I_{c1}=\tilde{I}_d\left(1-\frac{T}{\epsilon}\ln\frac{S_{e0}}{S_c}\right).
\label{E8}
\end{equation} 
For $S_c=10^2$ s$^{-1}$ used in our definition of $I_{sw}$, $S_{e0}=10^{12}$ s$^{-1}$, $\epsilon = 66$~K, and  $T = 0.9$~K, we get $I_{c1}\approx 0.69 \tilde{I}_d$, where $\tilde{I}_d=w\tilde{J}_d$. Such operational $I_{c1}$ equivalent to $I_{sw}$ is limited by the acceptable dark count rate $S_c$ and decreases logarithmically with the SNSPD length. The account of the extra factor $(1-J_s/\tilde{J}_d)$ in $S_{e0}$ only increases $I_{c1}$ by 3$\%$ and is neglected hereafter. 

\begin{figure}[h]
\centering
   	\includegraphics[scale=0.6,trim={0mm 0mm 0mm 0mm},clip]{supplementary/bueg.pdf}
   	\caption{Single vortices and antivortices penetrating from the film edges and vortex-antivortex pair unbinding inside the film due to thermal fluctuations.  }
   	\label{figE2}
   	\end{figure}
	
Consider now the critical current $I_{c2}$ limited by thermally-activated unbinding of VAV pairs inside the film. This process is illustrated in Fig.~\ref{figE2}, from which it follows that the energy scale for the VAV pair production is twice that of the vortices penetrating from the edges: 
\begin{equation}
U=2\epsilon\left(1-\frac{J_s}{J_d}\right),\qquad J_s\sim J_d.
\label{E9}
\end{equation}
This barrier vanishes at the bulk $J_d$ larger than $\tilde{J}_c$ for penetration of vortices from the edges. The VAV production rate in a film at $J_s\sim J_d$ can be evaluated in the same way as it was done above:
\begin{equation}
S_b=S_{b0}\exp\left[-\frac{2\epsilon}{T}\left(1-\frac{J_s}{J_d}\right)\right],\qquad S_{b0}\sim \frac{A\nu}{2\pi\xi_s^{2}}.
\label{E10}
\end{equation}
Here $A/2\pi\xi_s^2$ is a number of statistically-independent positions of the vortex core of size $\xi_s$ in a film of area $A$ and
\begin{equation}
S_{b0}\sim\frac{A\rho_n}{16\pi^2\mu_{0}\lambda_s^2\xi_s^{2}}. 
\label{E11}
\end{equation}
The critical current limited by the bulk VAV pair production is then
\begin{equation}
I_{c2}=I_{d}\left(1-\frac{T}{2\epsilon}\ln\frac{S_{b0}}{S_{c}}\right).
\label{E12}
\end{equation}
For $A=10\,\mu$m$\times 100\,\mu$m, $\rho_n=2.5\,\mu\Omega$m, $\lambda_s=950$~nm, $\xi_s=10$~nm, $\epsilon = 66$~K, and  $T = 0.9$~K, Eqs.~(\ref{E11}) and (\ref{E12}) give $S_{b0}\sim 1\cdot10^{17}\,s^{-1}$ and $I_{c2}\approx 0.76I_{d}$ at $S_c=10^2$ s$^{-1}$. Here $I_{c2}$ limited by the VAV unbinding decreases logarithmically with the SNSPD area.

As follows from Eqs.~(\ref{E7}) and (\ref{E12}), the logarithmic slopes of dark count rates for the VAV pair unbinding and the vortex hopping from the edges are related by:
\begin{equation}
\frac{d\ln S_b}{dI}=\left(\frac{2\tilde{J}_d}{J_d}\right)\frac{d\ln S_e}{d I}.
\label{E13}
\end{equation}
According to our experimental data shown in Fig.~1(d) in the main text, the slope $d\ln S/dI$ abruptly increases by a factor $1.79$ above a threshold current in the rails. This indicates switching from the dark counts limited by penetration of vortices from the edges to the bulk VAV pair unbinding. In this case Eq.~(\ref{E13}) can be used to evaluate the extent by which lithographic defects reduce the mean depairing current density at the edges: $\tilde{J}_d=0.895J_d$. Such relatively small decrease in $\tilde{J}_d$ is in line with the magnitude of reduction of $J(x)$ at the edges obtained in our numerical results shown in Fig.~\ref{figD2}(a).  

